Demystifying and Generalizing BinaryConnect

BinaryConnect (BC) and its many variations have become the de facto standard for neural network quantization. However, our understanding of the inner workings of BC is still quite limited. We attempt to close this gap in four different aspects: (a) we show that existing quantization algorithms, including post-training quantization, are surprisingly similar to each other; (b) we argue for proximal maps as a natural family of quantizers that is both easy to design and analyze; (c) we refine the observation that BC is a special case of dual averaging, which itself is a special case of the generalized conditional gradient algorithm; (d) consequently, we propose ProxConnect (PC) as a generalization of BC and we prove its convergence properties by exploiting the established connections. We conduct experiments on CIFAR-10 and ImageNet, and verify that PC achieves competitive performance.

==> img_neurips/failure_prox_quant.tex <==
% varepsilon = 0.02, a = 2.0
\begin{tikzpicture} [scale=0.4]
    \begin{axis}[samples=34, domain=-1:1, every axis plot/.append style={ultra thick}]
        \addplot +[mark=none] expression {x * (x > (0.02 - 1)) + ((1 - ((2 + 1) / 0.02)) * x + (1 + 2) * (1 - 50)) * (x <= (0.02 - 1))};
    \end{axis}
\end{tikzpicture}

==> sections/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{As discussed, the goal of our paper is to improve the understanding of BinaryConenct~\citep{courbariaux2015} and obtain novel generalizations. We therefore focus more on theory than empirical results. As a result, we only did extensive experiments on one dataset (CIFAR-10) with one architecture (ResNet20/56). As discussed in~\Cref{sec:imagenet}, our experiments on ImageNet are not exhaustive; both due to environmental reasons as well as limited availability of compute. In the future, we aim to do more exhaustive testing of ProxConnect (different architectures and problems), while keeping in mind the carbon footprint that comes with it.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See the first paragraph of~\Cref{sec:introduction}: quantization leads to decreased carbon footprint for training and inference (positive societal impact), however, it may come at the cost of increased bias (negative societal impact).}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are provided in the Appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We will provide the code once it has been approved by our internal process. We only ran experiments on publicly available datasets.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See~\Cref{sec:experiments},~\Cref{app:cifar10} and~\Cref{app:imagenet}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All experiments are over three random seeds; we provide mean and standard deviation for all results.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{The amount of compute in the exploration stage of our project was insignificant compared to the experiments reported in this work. See~\Cref{app:cifar10_gpu} and~\Cref{app:imagenet_gpu} for the total amount of compute we used for the experiments reported in this work.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See~\Cref{sec:cifar10} and~\Cref{sec:imagenet}.}
  \item Did you mention the license of the assets?
    \answerYes{Yes, the license of CIFAR-10 (MIT license) is included in the bibliography entry. The ImageNet dataset is ``is available for free to researchers for non-commercial use''.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We will provide the code once it has been approved by our internal process.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tabulars/fine.tex <==
\begin{tabular}{c | c | c c c}
    \toprule
    Model &  Quantization & BinaryConnect & ProxQuant & ProxConnect (Ours)\\
    \midrule
    ResNet20 & Binary & \textbf{90.31} (0.00) & 89.94 (0.10) & \textbf{90.31} (0.21)\\
    & Ternary & 74.95 (0.16) & \textbf{91.46} (0.06) & 91.37 (0.18)\\
    & Quaternary & 91.43 (0.07) & 91.43 (0.21) & \textbf{91.81} (0.14)\\
    \midrule
    ResNet56 & Binary & 92.22 (0.12) & 92.33 (0.06) & \textbf{92.65} (0.16)\\
    & Ternary & 74.68 (1.4) & 93.07 (0.02) & \textbf{93.25} (0.12)\\
    & Quaternary & 93.20 (0.06) & 92.82 (0.16) & \textbf{93.42} (0.12)\\
    \bottomrule
\end{tabular}

==> tabulars/methods.tex <==
%\tabulinesep =_1pt^1pt
\begin{tabular}{l c c c c c l}
    \toprule
    Method & PC & \faBolt &$\LP{\rho}$ &$\rho, \varrho$ &\faGraduationCap &$Q$\\
    \midrule
    ProxQuant-Binary-$L_1$~\citep{bai2018} &\xmark&\cmark &\cmark &$\shortarrow{1}$ &\xmark &$\{-1, 1\}$ \\
    ProxQuant-Ternary~\citep{bai2018}      &\xmark  &\xmark &\faDiamond       &$\shortarrow{1}$ &\xmark &$\{-1, 0, 1\}$\\
    \midrule
    BinaryConnect~\citep{courbariaux2015} &\cmark       &\cmark &\cmark &$\infty$         &\xmark &$\{-1, 1\}$ \\     
    BinaryRelax~\citep{yin2018}  &\cmark       &\cmark &\cmark &$0, \shortarrow{1}$ &\xmark &$\{-1, 1\}$\\
    BinaryWeight~\citep{rastegari2016}  &\cmark      &\cmark &\faDiamond      &$\infty$         &\cmark &$\{q_{j,1}, q_{j,2}\}$\\
    MirrorDescentView~\citep{ajanthan2021}  &\cmark     &\cmark &\faSkyatlas &- &\xmark &$\{-1, 1\}$ \\
    TrainedTernary\textsuperscript{\textdagger}~\citep{zhu2016} &\cmark     &\cmark &\cmark &$\infty$         &\cmark &$\{q_{j,1}, 0, q_{j,2}\}$ \\
    TernaryWeight\textsuperscript{\textdagger}~\citep{li2016arxiv}  &\cmark    &\cmark &\faDiamond      &$\infty$         &\cmark &$\{-q_{j,1}, 0, q_{j,1}\}$ \\
    %\midrule
    %\tabucline[0.4pt off 2pt]{-}
    \midrule
    ProxConnect (ours)  &-    &\cmark &\cmark &$\shortarrow{1}$ &\cmark &$Q_j$ \\
    \bottomrule
\end{tabular}

==> tabulars/methods_revised_old.tex <==
%\tabulinesep =_1pt^1pt
\begin{tabular}{l c c c c c l}
    \toprule
    Method & PC & One-pass &Learned parameters &$\LP{\rho}$ &$\rho, \varrho$ & $Q$\\
    \midrule
    ProxQuant-Binary-$L_1$~\citep{bai2018} &\xmark &\cmark &\xmark &\cmark &$\shortarrow{1}$ &$\{-1, 1\}$ \\
    ProxQuant-Ternary~\citep{bai2018}      &\xmark &\xmark &\xmark &\xmark      &-  &$\{-1, 0, 1\}$\\
    \midrule
    BinaryConnect~\citep{courbariaux2015} &\cmark &\cmark      &\xmark &\cmark &$\infty$          &$\{-1, 1\}$ \\     
    BinaryRelax~\citep{yin2018}  &\cmark       &\cmark &\xmark &\cmark &$0, \shortarrow{1}$  &$\{-1, 1\}$\\
    BinaryWeight~\citep{rastegari2016}  &\cmark      &\cmark &\cmark &\xmark      &-          &$\{q_{j,1}, q_{j,2}\}$\\
    MirrorDescentView~\citep{ajanthan2021}  &\cmark     &\cmark &\xmark &\xmark &-  &$\{-1, 1\}$ \\
    TrainedTernary\textsuperscript{\textdagger}~\citep{zhu2016} &\cmark     &\cmark &\cmark &\cmark &$\infty$          &$\{q_{j,1}, 0, q_{j,2}\}$ \\
    TernaryWeight\textsuperscript{\textdagger}~\citep{li2016arxiv}  &\cmark    &\cmark &\cmark &\xmark      &-        &$\{-q_{j,1}, 0, q_{j,1}\}$ \\
    %\midrule
    %\tabucline[0.4pt off 2pt]{-}
    \midrule
    ProxConnect (ours)  &-    &\cmark &\cmark &\cmark &$\shortarrow{1}$ &$Q_j$ \\
    \bottomrule
\end{tabular}
